Discovery of a Metal-Poor Red Giant Star with the Highest Ultra-Lithium Enhancement

We present the discovery of 2MASS J05241392-0336543 (hereafter J0524-0336), a very metal-poor ([Fe/H]=-2.43 +- 0.16), highly r-process-enhanced ([Eu/Fe]= +1.34 +- 0.10) Milky Way halo field red giant star, with an ultra high Li abundance of A(Li)(3D,NLTE)= 6.15 +- 0.25 and [Li/Fe]= +7.64 +- 0.25, respectively. This makes J0524-0336 the most lithium-enhanced giant star discovered to date. We present a detailed analysis of the star's atmospheric stellar parameters and chemical abundance determinations. Additionally, we detect indications of infrared excess, as well as observe variable emission in the wings of the H_alpha absorption line across multiple epochs, indicative of a potential enhanced mass-loss event with possible outflows. Our analysis reveals that J0524-0336 lies either between the bump and the tip of the Red Giant Branch (RGB), or on the early-Asymptotic Giant Branch (e-AGB). We investigate the possible sources of lithium enrichment in J0524-0336, including both internal and external sources. Based on current models and on the observational evidence we have collected, our study shows that J0524-0336 may be undergoing the so-called lithium flash that is expected to occur in low-mass stars when they reach the RGB bump and/or the early-AGB.

==> LightAbundances.tex <==
%delete X/Fe err convert all tables to deluxe table format
%Add Synthesis elements to table (All abundances in one table)
%2tables, average abundances (use synth abundances from graphs I made), and we need linelist (every single line, extract all lines from smh and include, NOT chem abund.) 
%\begin{table}
\begin{deluxetable*} {c c c c c c c c} 
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:ident} Light Element Abundances}
\tablehead{
\colhead{El} & \colhead{N} & \colhead{log(X)$_{\odot}$} & \colhead{log(X)} & \colhead{[X/H]} & \colhead{[X/Fe]} & \colhead{$\sigma$[X/H]} &}
\startdata 
Li (Syn.) & 7   & +1.05 & +6.16    & +5.11   & +7.67   & \nodata    \\  
C (Syn.)  & 1   & $+8.43$ & +0.00    & -8.43   & -5.88   & 0.10     \\
\nai      & 2   & +6.24 & +5.24    & -1.00   & +1.55   & 0.06       \\
\oi       & 1   & +8.69 & +7.37    & -1.32   & +1.23   & \nodata      \\
\mgi      & 7   & +7.60 & +5.47    & -2.13   & +0.43   & 0.09       \\
\ali      & 1   & +6.45 & +2.01    & -4.44   & -1.89   & \nodata    \\
\sii      & 2   & +7.51 & +5.65    & -1.86   & +0.70   & 0.08       \\
\ki       & 2   & +5.03 & +3.03    & -2.00   & +0.56   & 0.01       \\
\cai      & 21  & +6.34 & +4.07    & -2.27   & +0.28   & 0.13       \\
%Sc I      & 1   & +3.15 & +2.98    & -0.17   & +2.38   & \nodata   \\
\scii     & 11  & +3.15 & +0.82    & -2.33   & +0.23   & 0.09       \\
%Ti I      & 30  & +4.95 & +2.63    & -2.32   & +0.23   & 0.15      \\
\tiii     & 43  & +4.95 & +2.72    & -2.23   & +0.32   & 0.17       \\
%V I       & 1   & +3.93 & +4.47    & +0.54   & +3.09   & \nodata   \\
%V II      & 1   & +3.93 & +1.81    & -2.12   & +0.43   & \nodata   \\
\cri      & 16  & +5.64 & +3.02    & -2.62   & -0.07   & 0.09       \\
\crii     & 2   & +5.64 & +3.29    & -2.35   & +0.20   & 0.19       \\
\mni      & 4   & +5.43 & +2.58    & -2.85   & -0.30   & 0.04       \\
\fei      & 178 & +7.50 & +4.95    & -2.55   & +0.00   & 0.24       \\
\feii     & 17  & +7.50 & +4.95    & -2.55   & +0.01   & 0.16       \\
\coi      & 4   & +4.99 & +2.25    & -2.74   & -0.19   & 0.06       \\
\nii      & 16  & +6.22 & +3.64    & -2.58   & -0.03   & 0.16        \\
\zni      & 2   & +4.56 & +1.99    & -2.57   & -0.02   & 0.02       \\     
\enddata
\end{deluxetable*}
%\end{table}
%must do abundance error analysis 
%include SD from plots I made for synth data

==> lum.tex <==
\begin{deluxetable*} {c c c} 
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:ident} Light Element Abundances}
\tablehead{
\colhead{property} & \colhead{value} & \colhead{error}}
Lum(L\odot) & 155.4 & 
    \\  

         \\     
\enddata
\end{deluxetable*}

==> photemp.tex <==
\begin{deluxetable}{ c c c}
\tablewidth{0pt}
\tabletypesize{\footnotesize}
\tablecaption{\label{tab:pho} Photometric Temperature Calculations from Different Bands}
\tablehead{
\colhead{Photometric Color} & \colhead{\teff\ (K)} & \colhead{$\sigma$\,\teff}(K)}
\startdata
(B-R) & 3894 & 64     \\
(R-J) & 4730 & 93  \\
(R-H) & 4687 & 59  \\
(R-K) & 4696 & 46   \\
(B-J) & 3917 & 49   \\
(B-H) & 3959 & 40  \\
(B-K) & 4014 & 33  \\ 
(G-J) & 4169 & 56  \\
(G-H) & 4309 & 41  \\
(G-K) & 4286 & 31     \\
Mean & 4279 & 51.2   \\
\enddata
\end{deluxetable}
